3D-Assisted Image Feature Synthesis for Novel Views of an Object

Comparing two images in a view-invariant way has been a challenging problem in computer vision for a long time, as visual features are not stable under large view point changes. In this paper, given a single input image of an object, we synthesize new features for other views of the same object. To accomplish this, we introduce an aligned set of 3D models in the same class as the input object image. Each 3D model is represented by a set of views, and we study the correlation of image patches between different views, seeking what we call surrogates --- patches in one view whose feature content predicts well the features of a patch in another view. In particular, for each patch in the novel desired view, we seek surrogates from the observed view of the given image. For a given surrogate, we predict that surrogate using linear combination of the corresponding patches of the 3D model views, learn the coefficients, and then transfer these coefficients on a per patch basis to synthesize the features of the patch in the novel view. In this way we can create feature sets for all views of the latent object, providing us a multi-view representation of the object. View-invariant object comparisons are achieved simply by computing the $L^2$ distances between the features of corresponding views. We provide theoretical and empirical analysis of the feature synthesis process, and evaluate the proposed view-agnostic distance (VAD) in fine-grained image retrieval (100 object classes) and classification tasks. Experimental results show that our synthesized features do enable view-independent comparison between images and perform significantly better than traditional image features in this respect.

==> related.tex <==
shape features


Such representation [list a number of advantages, 1. effective for shape retrieval in SHREC challenges, 2. efficient to compute and store]. More importantly, it allows us to bypass the highly challenging task of reconstructing geometric structures or high-fidelity novel view images, but still preserves rich information in feature space for many kinds of image recognition and comparison tasks.


view-invariant image features;

local subspace embedding;

transfer-learning;

graph structure learning;	

3D reconstruction;	

shape descriptor \& distance;

traditional image search/comparison	;

query expansion;


If a shape collection does include the exact shape of the imaged object, then the solution is as simple as finding that shape and then adopting its shape descriptor. Recent work such as \cite{Aubry14,lim2013parsing} follows such exemplar-based scheme. However, such approaches assume a large-scale shape collection, whereas 2D images are still many orders of magnitudes more than 3D shapes in diversity and quantity.

We aim for shape descriptor reconstruction using modestly-sized shape network. To achieve the goal, rather than viewing existing shapes as individuals, we use them together to build a shape descriptor space. In this way, we can ``interpolate'' the descriptor of the \emph{latent shape}, which amounts to synthesizing features at novel views by interpolation using existing shapes. To be more concrete, for each patch in the novel view, its feature can be reconstructed by interpolation using the same patch from other shapes at the same view.


==> representation.tex <==
\label{sec:ShapeRepresentation}
{\color{blue}
	what is render-based shape representation;
	
	why choose this representation;
}



The shape representation in this paper is render-based, which is also known as 2.5D shape descriptor [CITE SILVIO]. In words, a shape is represented as a network of patch-based image features from different views. To be more precise, we render images from different viewpoints and extract {\bf patch-based} features for each image, such as HoG or Deep Learning features\footnote{output from lower level convolutional layers, blablabla}. \emph{So we focus on the reconstruction of 2.5D shape descriptor, rather than the shape itself.} 

Such representation [list a number of advantages, 1. effective for shape retrieval in SHREC challenges, 2. efficient to compute and store]. More importantly, it allows us to bypass the highly challenging task of reconstructing geometric structures or high-fidelity novel view images, but still preserves rich information in feature space for many kinds of image recognition and comparison tasks.


